Scalable Unsupervised Multi-Criteria Trajectory Segmentation and Driving Preference Mining

We present analysis techniques for large trajectory data sets that aim to provide a semantic understanding of trajectories reaching beyond them being point sequences in time and space. The presented techniques use a driving preference model w.r.t. road segment traversal costs, e.g., travel time and distance, to analyze and explain trajectories. In particular, we present trajectory mining techniques that can (a) find interesting points within a trajectory indicating, e.g., a via-point, and (b) recover the driving preferences of a driver based on their chosen trajectory. We evaluate our techniques on the tasks of via-point identification and personalized routing using a data set of more than 1 million vehicle trajectories collected throughout Denmark during a 3-year period. Our techniques can be implemented efficiently and are highly parallelizable, allowing them to scale to millions or billions of trajectories.

==> appendices/acmp-details.tex <==
\section{Number of Wrong Turns}\label{app:number-of-wrong-turns}
The algorithm to compute the number of wrong turns (see \cref{sec:robust-driving-preference-recovery}) is given below. Here, $(v_i,v_{i+1})$ denotes the edge from node $v_i$ to node $v_{i+1}$.
\begin{algorithm}
	\caption{Number of Wrong Turns \label{alg:wt}}
	
	\begin{algorithmic}[1]
		\Function{WT}{$\pi(s,t)=(s=v_0,v_1,\dots,v_{k-1},t=v_k),\alpha$}
		\State $wt \gets 0$
		\For{$i$ \textbf{from} $0$ \textbf{to} $k-1$}
		\State $\pi' \gets \text{getShortestPath}(v_i,t,\alpha)$
		\If{$(v_i,v_{i+1})\notin \pi'$}
		\State $wt \gets wt + 1$
		\EndIf
		\EndFor
		\State \Return $wt$
		\EndFunction
	\end{algorithmic}
\end{algorithm}


==> appendices/break-recovery-rate-correlations.tex <==
\section{Additional Figures for Single-Metric Trajectory Segmentation Experiments}\label{app:single-metric-figures}
\begin{figure}
   \centering
   \includegraphics[width=\linewidth]{figures/travel-time-metric-segmentation-window-brr-distribution.png}
  \caption{Distribution of within-window \ac{brr} for single-metric trajectory segmentation.\label{fig:single-metric-brr-window-dist}}
\end{figure}


\cref{fig:single-metric-scatter-plots} show how exact and within-window \ac{brr} changes depending on trajectory length and the number of breaks in a trajectory.
Note that the symmetry at a low number of breaks in \cref{fig:single-metric-scatter-plots-b,fig:single-metric-scatter-plots-d} is a consequence of the \ac{brr} only being able to take a finite number of values equal to the number of breaks.

\begin{figure*}[h]
  \begin{subfigure}{0.495\textwidth}
     \includegraphics[width=\linewidth]{%
       figures/travel-time-metric-segmentation-exact-brr-vs-trajectory-length.png}
       \caption{}
  \end{subfigure}
  \begin{subfigure}{0.495\textwidth}
   \includegraphics[width=\linewidth]{%
     figures/travel-time-metric-segmentation-exact-brr-vs-no-of-stitches.png}
       \caption{\label{fig:single-metric-scatter-plots-b}}
  \end{subfigure}

  \begin{subfigure}{0.495\textwidth}
     \includegraphics[width=\linewidth]{%
       figures/travel-time-metric-segmentation-within-window-brr-vs-trajectory-length.png}
       \caption{}
  \end{subfigure}
  \begin{subfigure}{0.495\textwidth}
     \includegraphics[width=\linewidth]{%
       figures/travel-time-metric-segmentation-within-window-brr-vs-no-of-stitches.png}
       \caption{\label{fig:single-metric-scatter-plots-d}}
  \end{subfigure}
  \caption{Changes in (a, b) exact \ac{brr} and (c, d) within-window \ac{brr} for single-metric trajectory segmentation as a function of either (a, c) the length of a trajectory or (b, d) the number of breaks in a trajectory.\label{fig:single-metric-scatter-plots}}
\end{figure*}


\section{Additional Figures for Multi-Metric Trajectory Segmentation Experiments}\label{app:multi-metric-figures}
\begin{figure}
   \includegraphics[width=\linewidth]{%
     figures/four-metrics-segmentation-exact-brr-distribution.png}
\end{figure}

\begin{figure}
   \includegraphics[width=\linewidth]{%
     figures/four-metrics-segmentation-exact-brr-vs-no-of-stitches.png}
\end{figure}


\begin{figure}
   \includegraphics[width=\linewidth]{%
     figures/four-metrics-segmentation-exact-brr-vs-trajectory-length.png}
\end{figure}



\begin{figure}
   \includegraphics[width=\linewidth]{%
     figures/four-metrics-segmentation-window-brr-distribution.png}
\end{figure}

\begin{figure}
   \includegraphics[width=\linewidth]{%
     figures/four-metrics-segmentation-within-window-brr-vs-no-of-stitches.png}
\end{figure}

\begin{figure}
   \includegraphics[width=\linewidth]{%
     figures/four-metrics-segmentation-within-window-brr-vs-trajectory-length.png}
\end{figure}





\begin{figure*}[h]
  \begin{subfigure}{0.495\textwidth}
     \includegraphics[width=\linewidth]{%
       figures/four-metrics-segmentation-exact-brr-vs-trajectory-length.png}
       \caption{}
  \end{subfigure}
  \begin{subfigure}{0.495\textwidth}
   \includegraphics[width=\linewidth]{%
     figures/four-metrics-segmentation-exact-brr-vs-no-of-stitches.png}
       \caption{}
  \end{subfigure}

  \begin{subfigure}{0.495\textwidth}
     \includegraphics[width=\linewidth]{%
       figures/four-metrics-segmentation-within-window-brr-vs-trajectory-length.png}
       \caption{}
  \end{subfigure}
  \begin{subfigure}{0.495\textwidth}
     \includegraphics[width=\linewidth]{%
       figures/four-metrics-segmentation-within-window-brr-vs-no-of-stitches.png}
       \caption{}
  \end{subfigure}
  \caption{Changes in (a, b) exact \ac{brr} and (c, d) within-window \ac{brr} for multi-metric segmentation as a function of either (a, c) the length of a trajectory or (b, d) the number of breaks in a trajectory.\label{fig:multi-metric-scatter-plots}}
\end{figure*}


\begin{figure}
   \includegraphics[width=\linewidth]{%
     figures/four-metrics-segmentation-window-brr-distribution.png}
\end{figure}







==> brr_single_metric_experiments_old.tex <==

We use several measures to assess the quality trajectory decomposition.
We measure the \emph{\ac{brr}} of each trajectory.
Let $D_T$ be the trajectory decomposition of trajectory $T$ with break points $B_T$.
The \ac{brr} of trajectory decomposition $D_T$ is defined as
\begin{equation}
  \mathit{BRR}(D_T) = \sum_{b \in B_T} \frac{[b \in D_T]}{|B_T|},
\end{equation}
where $[b \in D_T]$ has a value of one if $b \in D_T$, otherwise it has a value of zero.
The \ac{brr} measures exact recovery of the break point where a decomposition point has exactly the same position as the break point.
However, the decomposition algorithm often has a decomposition window where a decomposition point can be placed arbitrarily without changing the correctness and optimality of the decomposition w.r.t.\ the amount of segments created.
We therefore consider both exact and within-window \ac{brr}.

In the cases where break points are not recovered, we are interested in seeing how far off the break points are.
\TODO{Tobias: Finish distance and window tightness.}
We are interested in marking interesting spots along the trajectory (stitches, in this case), as accurately as possible.
We have therefore also examined the tightness of the windows in within-window stitch recovery, i.e, the number of edges the windows of a decomposed trajectory contain on average.



\begin{table}
  \centering
  \caption{Results for Exact and Within-Window Stitch Recovery for Decomposition using only the Travel Time Metric.\label{tab:one-metric-stitch-recovery}}
  \begin{tabular}{lcc}
    \toprule
     & \emph{Exact} & \emph{Within-Window} \\
    \midrule
    Recovered & $0.38$ & $0.42$ \\  % 0.3815238096637161 & 0.4209375298738193
    Tightness & $1.00$ & $1.19$ \\  % 1.1941858873201343
    Distance  & $2.30$ & $1.20$ \\  % 2.3021841987105716$ & $1.199136773217926$
    \bottomrule
  \end{tabular}
\end{table}


As can be seen in \cref{tab:one-metric-stitch-recovery}, our proposed decomposition method recovers on average $38\%$ and $42\%$ of breaks in a trajectory, using exact and within-window break recovery, respectively.
However, the increase in break recovery is off-set by an increase in tightness on the break-recovering segmentation windows.
In other words, the windows recover more breaks, but the windows tend to be less informative than the segmentation points.
Similarly, the unrecovered breaks tend to be nearer an edge of a segmentation window than a segmentation point, with an average distance of $1.20$ edges to segmentation windows and an average distance of $2.30$ edges to segmentation points.


The distribution of the \acp{brr}, shown for exact \ac{brr} in \cref{fig:single-metric-brr-exact-dist}, reveals that no breaks are recovered at all for a large proportion of the trajectories. 
The distribution for within-window \ac{brr} shows a similar pattern, see \cref{fig:single-metric-brr-window-dist} in \cref{app:single-metric-figures}.
This skew is explained by the trajectory segmentation method's failure to divide $65\,216$ of the trajectories.
The trajectories that were not divided during trajectory segmentation have been excluded from the calculation of the distances in \cref{tab:one-metric-stitch-recovery}.

We found only a weak tendency for \ac{brr} to lower as trajectory length (in number of edges), and the number of breaks in a trajectory increases, with Pearson correlation values of $r=-0.21$, and $r=-0.18$ for exact \ac{brr}, respectively.
We show these relationships in further details plots in \cref{fig:single-metric-scatter-plots} in \cref{app:single-metric-figures}.

We have also examined the ratio of segmentation points and windows to recovered breaks which are $4.25:1$ and $3.78:1$ for exact break recovery and within-window break recovery, respectively.
In other words, about one-fifth of the trajectory segments given by the trajectory segmentation algorithm signify a break.
However, since our data only contains positive examples of interesting behavior within the trajectory (breaks, in our dataset), we cannot determine whether the trajectory segments that do not match a break are false positives or signify some other interesting, but unknown, behavior during the trajectory.

\ignore{
\TODO{Florian/Tobias}
Report sizes of UMS and SPS (in particular compare to single criteria segmentation):
\begin{itemize}
	\item for all unstitched trajectories: report average/max number of pieces
	\item for all stitched trajectories: report average/max number of pieces
	\item detailed analysis of stitch recovery: how many real stitch points are identified (exactly or nearby) -- how many breakpoints correspond to actual stitch points (exactly or nearby)? 
\end{itemize}
Probably it also makes sense to do all this for each metric separately for comparison and then for the conic combination variant. Aggregate where necessary not to create too many redundancies with last section.
\TODO{Tobias?}
Report on:
\begin{itemize}
	\item for all unstitched trajectories: report average/max number of pieces
          \COMMENT{Tobias}{These statistics seem irrelevant for this experiment?}
	\item for all stitched trajectories: report average/max number of pieces
      % Mean Trajectory Length: 287.6992198009147 edges.
      % Max Trajectory Length: 12456 edges.
      % Mean No. of Stitches: 4.020915484838003 stitches.
      % Max No. of Stitches: 174 stitches.
	\item detailed analysis of stitch recovery: how many real stitch points are identified (exactly or nearby) -- how many breakpoints correspond to actual stitch points (exactly or nearby)? 
\end{itemize}
}


==> data.tex <==
\relax 
\providecommand\hyper@newdestlabel[2]{}


==> data_description_.tex <==
\section{Data Description}

\subsection{Costs}

\subsubsection{Travel Time}
Travel times are derived from a combination of observed driving speeds and historical driving speeds.
The travel time $t_s$ for a road segment $s$ is
\begin{equation}
  t_s = l_s / d_s
\end{equation}
where $l_s$ is the length of segment $s$, and $d_s$ is the driving speed on segment $d_s$.
For all road segments $s \in S$, we derive the driving speed based on an estimate of the mean driving speed on segment $s$ and a set of historical driving speeds observed from traversals in the trajectory data set. Specifically, we compute $d_s$ as a weighted mean
\begin{equation}
  d_s = \frac{k*\hat{d_s} + n*\bar{d_s}}
             {k+n}
\end{equation}
where $\hat{d_s}$ is the estimate of the mean driving speed, $\bar{d_s}$ is the mean driving speed derived from the set of historical trajectories, $n$ is the number of historical traversals of segment $s$ in the trajectory dataset, and $k$ represents the confidence in $\hat{d_s}$.
This approach ensures that the travel time estimate is robust to outliers when there are only a few observations but also that travel time estimates can be assigned even for segments without any historical trajectories.

\paragraph{Mean Driving Speed Estimation}
\begin{itemize} 
  \item Inferred driving speeds cannot be below 5 kmh.
  \item Use $k=10$ based on previous work (see some of CSJ papers)
  \item Perhaps some stats on the mean absolute error?
\end{itemize}

\subsubsection{Normalization}

Before normalization:
\begin{itemize}
  \item travel time has mean 50.380633987049166 with a range of [0.0; 2338.76416015625].
  \item crowdedness has mean 0.018450799966840806 with a range of [0.0; 1.0].
  \item congestion has mean 0.7688636713322032 with a range of [0; 0.9720605547939029].
  \item unit distance has mean 1.0 with a range of [1.0; 1.0].
\end{itemize}

After normalization:
\begin{itemize}
  \item travel time has mean 0.9999999999999997 with a range of [0.0; 46.42188823502003].
  \item crowdedness has mean 1.0000000000000002 with a range of [0.0; 54.19819204571988].
  \item congestion has mean 1.0000000000000002 with a range of [0.0; 1.264282071111022].
  \item unit distance has mean 1.0 with a range of [1.0; 1.0].
\end{itemize}


==> temp.tex <==



==> tmp.tex <==
\begin{abstract}
	We examine a large corpus of real-world trajectories  and develop analysis techniques in order to obtain a better understanding of the trajectories reaching further than mere point sequences in time and space. The main ingredient of our techniques is the investigation how well given network metrics like travel time, distance, or a combination thereof are able to explain a trajectory. Based on that we can analyze single trajectories as well as trajectory collections with respect to similarity in their driving preferences.  
	For our concrete data set of more than 1 million vehicle trajectories collected throughout Denmark during a 3-year period, we perform an extensive experimental investigation both for single trajectories as well as trajectory sets and multiple metrics.  
\end{abstract}


==> travel_time_.tex <==
\section{Metric Details}
In this section, we describe how the travel time, congestion, and crowdedness metrics are derived in further details.

\subsection{Travel Time}\label{sec:travel-time-derivation}
The vehicle trajectories in our trajectory set have tendency to be concentrated on a few popular segments, as such, many road segments have few or no traversals in the trajectory set.
We therefore require a means of estimating travel times for such road segments.
However, for road segments with an abundance of traversal data such an estimate may be inaccurate.
Inspired by previous work~\cite{estimation-updates}, we therefore combine travel time estimates with travel times of historical traversals s.t.\ when the driving speed estimate of a road segment becomes increasingly less influential the more historical traversals the road segment is associated with.

We compute the travel time $t_e$ for a road segment $e$ as
\begin{equation}\label{eq:travel-time-derivation}
  t_e = \frac{k*\hat{t_e} + n*\bar{t_e}}
             {k+n}
\end{equation}
where $\hat{t_e}$ is the estimate of the mean travel time, $\bar{t_e}$ is the mean travel time of the historical traversals, $n$ is the number of historical traversals of segment $e$ in the trajectory dataset, and $k$ represents the confidence in $\hat{t_e}$.

\TODO{Tobias: Should reference currently unpublished paper, but can put version on ArXiV.}
We use a pre-trained \ac{rfn}~\cite{rfn-short} to provide travel time estimates $\hat{t_e}$ for each road segment $e \in E$.
Specifically, we use the best performing \ac{rfn} from~\cite{rfn-short} which has been trained on the Danish Municipality of Aalborg using trajectories within the municipality that occurred between January 1 2012 and June 30 2013. Despite having been trained only on a subset of the network, the model generalizes well to unseen areas of the road network~\cite{rfn-long}. However, in a few cases the network would give very low values. We therefore modify the output s.t.\ the estimated driving speed on any road segment cannot be below $5$ kmh.



==> working-glossary.tex <==
Agreed upon glossary:
\begin{description}
  \item[Trajectory] Refers to paths or routes in the road network that were generated based on GPS data.
  \item[Path] Refers to (shortest) paths used in algorithms. Are of a theoretical or hypothetical nature, rather than from real data.
  \item[(Trajectory) Segmentation] Refers to the process of partitioning a trajectory into segments.
  \item[A (Trajectory) Segmentation] Is a collection of segmentation points that result from the process of trajectory segmentation.
  \item[Segmentation Point] Refers to the points in a trajectory that mark the start of a new segment of the trajectory.
  \item[Cost Functions] Assigns cost values to segments or routes. Used in place of metric.
  \item[Cost(s)] Concrete cost vector values.
  \item[stitch point] REAL location where something happend (gas station ...)
  \item[break point] sometimes synonomous with segmentation point, sometimes nearly-synonomous with stitch point; need to unify at some point
\end{description}


==> working_glossary.tex <==
Agreed upon glossary:
\begin{description}
  \item[Trajectory] Refers to paths or routes in the road network that were generated based on GPS data.
  \item[Path] Refers to (shortest) paths used in algorithms. Are of a theoretical or hypothetical nature, rather than from real data.
  \item[(Trajectory) Segmentation] Refers to the process of partitioning a trajectory into segments.
  \item[A (Trajectory) Segmentation] Is a collection of segmentation points that result from the process of trajectory segmentation.
  \item[Segmentation Point] Refers to the points in a trajectory that mark the start of a new segment of the trajectory.
\end{description}


